Quantum nonergodicity and fermion localization in a system with a single-particle mobility edge

We study the many-body localization aspects of single-particle mobility edges in fermionic systems. We investigate incommensurate lattices and random disorder Anderson models. Many-body localization and quantum nonergodic properties are studied by comparing entanglement and thermal entropy, and by calculating the scaling of subsystem particle number fluctuations, respectively. We establish a nonergodic extended phase as a generic intermediate phase (between purely ergodic extended and nonergodic localized phases) for the many-body localization transition of non-interacting fermions where the entanglement entropy manifests a volume law (`extended'), but there are large fluctuations in the subsystem particle numbers (`nonergodic'). We argue such an intermediate phase scenario may continue holding even for the many-body localization in the presence of interactions as well. We find for many-body states in non-interacting 1d Aubry-Andre and 3d Anderson models that the entanglement entropy density and the normalized particle-number fluctuation have discontinuous jumps at the localization transition where the entanglement entropy is sub-thermal but obeys the "volume law". In the vicinity of the localization transition we find that both the entanglement entropy and the particle number fluctuations obey a single parameter scaling. We argue using numerical and theoretical results that such a critical scaling behavior should persist for the interacting many-body localization problem with important consequences. Our work provides persuasive evidence in favor of there being two transitions in many-body systems with single-particle mobility edges, the first one indicating a transition from the purely localized nonergodic many-body localized phase to a nonergodic extended many-body metallic phase, and the second one being a transition eventually to the usual ergodic many-body extended phase.

==> notes_ReturnProb.tex <==
\subsection{Return probability of quantum states} 
\label{subsec:returnprob} 
Another useful quantity to track the localization transition is the quantum return probability (QRP), which directly captures the capability of preserving quantum information of a many-body localized system. In calculating the return probability, we take an initial product state 
\be 
|\Psi_{\rm init} \rangle =   c_{j_1} ^\dag c_{j_2 } ^\dag \ldots c_{j_N} ^\dag |{\rm vac} \rangle 
% (c_1 ^\dag ) ^{n_1} (c_2 ^\dag )^{n_2} \ldots (c_{D} ^\dag) ^{n_D} |{\rm vac}\rangle, 
\ee 
and evaluate the wavefunction overlap between the time-evolved and initial states, 
\be 
{\rm QRP} (t) = | \langle \Psi (t ) | \Psi_{\rm init} \rangle |^2. 
\ee 
In the non-interacting case,  the time-evolved state $|\Psi (t)\rangle$ is 
\be 
|\Psi (t) \rangle =  c_{j_1 } ^\dag (t ) c_{j_2 } ^\dag (t) \ldots c_{j_N} ^\dag (t) | {\rm vac} \rangle 
%  [c_1 ^\dag (t) ] ^{n_1} [c_2 ^\dag  (t) ]^{n_2} \ldots [c_{D} ^\dag (t) ] ^{n_D} |{\rm vac}\rangle, 
\ee 
with 
$c_j ^\dag (t) = e^{-i H_0 t} c_j ^\dag  e^{i H_0 t} = \sum_{\alpha, j'}   \phi_\alpha  ^* (j)   \phi_\alpha (j')  e^{-i \epsilon_\alpha t} 
c_{j'} ^\dag  $. 
The wave function overlap is then given by the determinant of the matrix 
\be 
{\cal M}_{i  i'} = \sum_{\alpha}   \phi_\alpha  ^* (j_i )   \phi_\alpha (j_{i'} )  e^{-i \epsilon_\alpha t}, 
\ee 
with $1\le i\le N$. 

With a extended Hamiltonian, the QRP approaches zero quickly (exponential in time), and  the quantum information becomes completely delocalized in Fock space.  At long time, the QRP in the ergodic system is expected to approach $1/V_H$. With a localized non-interacting Hamiltonian the  QRP  approaches to a finite value at long time, as the quantum information is not able to spread over the Fock space. For an interacting system, the QRP is expected to always  approach zero at long time, but in a power-law fashion, which is different from the extended phase.  
